Caramel: Accelerating Decentralized Distributed Deep Learning with Computation Scheduling

The method of choice for parameter aggregation in Deep Neural Network (DNN) training, a network-intensive task, is shifting from the Parameter Server model to decentralized aggregation schemes (AllReduce) inspired by theoretical guarantees of better performance. However, current implementations of AllReduce overlook the interdependence of communication and computation, resulting in significant performance degradation. In this paper, we develop Caramel, a system that accelerates decentralized distributed deep learning through model-aware computation scheduling and communication optimizations for AllReduce. Caramel achieves this goal through (a) computation DAG scheduling that expands the feasible window of transfer for each parameter (transfer boundaries), and (b) network optimizations for smoothening of the load including adaptive batching and pipelining of parameter transfers. Caramel maintains the correctness of the dataflow model, is hardware-independent, and does not require any user-level or framework-level changes. We implement Caramel over TensorFlow and show that the iteration time of DNN training can be improved by up to 3.62x in a cloud environment.

==> common/common-acm.tex <==
\settopmatter{printacmref=false}
\renewcommand\footnotetextcopyrightpermission[1]{}
\pagestyle{plain}
\input{./common/common}
\newcommand\xdiv[2]{\opexpr{#1/#2}{sol}\opround{sol}{0}{sol}\opprint{sol}}

==> common/common.tex <==
%\usepackage[margin=1in]{geometry} 
\usepackage{subcaption}
\usepackage{amsmath,amsthm,amssymb, graphicx,array}
%\usepackage{mathtools}
%\usepackage[scientific-notation=true]{siunitx}
%\usepackage{wrapfig}
\usepackage{xspace}
%\sisetup{detect-all}
%\sisetup{output-exponent-marker=\ensuremath{\mathrm{E}}}
\def\snum#1{\num[round-precision=3,round-mode=figures]{#1}} 
\def\xparagraph#1{\vspace{5pt}\noindent\textbf{#1}: }
%\usepackage[final]{listings}
%\usepackage{color}
%\usepackage[dvipsnames]{xcolor}
%\usepackage{multicol}
%\usepackage{multirow}
%\usepackage{hyperref}
%\usepackage{glossaries}
%\usepackage{nomencl}
%\usepackage{subcaption}
%\usepackage[hypcap=true]{caption}
%\usepackage{pgfplots}
%\usepackage[linesnumbered,lined,ruled]{algorithm2e}
%\usepackage{csvsimple}
%\usepackage[all]{xy}
%\usepackage{floatrow}
%\usetikzlibrary{patterns}
%\usepgfplotslibrary{colorbrewer}
%\pgfplotsset{compat=newest}
%\usepgfplotslibrary{groupplots}

\definecolor{dkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}

\lstset{frame=tb,
  language=C++,
  aboveskip=3mm,
  belowskip=3mm,
  showstringspaces=false,
  columns=flexible,
%  basicstyle={\small\ttfamily},
  numbers=left,
%  numberstyle=\small\color{gray},
  keywordstyle=\color{blue},
  commentstyle=\color{dkgreen},
  stringstyle=\color{mauve},
  breaklines=true,
  breakatwhitespace=true,
  tabsize=4
}

% \lstdefinelanguage{Ini}
% {
%     basicstyle=\ttfamily\small,
%     columns=fullflexible,
%     morecomment=[s][\color{blue}\bfseries]{[}{]},
%     morecomment=[l]{\#},
%     morecomment=[l]{;},
%     commentstyle=\color{gray}\ttfamily,
%     morekeywords={},
%     otherkeywords={=,:},
%     keywordstyle={\color{black}\bfseries}
% }

%\pgfplotsset{
%    discard if/.style 2 args={
%        x filter/.code={
%            \edef\tempa{\thisrow{#1}}
%            \edef\tempb{#2}
%            \ifx\tempa\tempb
%                \def\pgfmathresult{inf}
%            \fi
%        }
%    },
%    discard if not/.style 2 args={
%        x filter/.code={
%            \edef\tempa{\thisrow{#1}}
%            \edef\tempb{#2}
%            \ifx\tempa\tempb
%            \else
%                \def\pgfmathresult{inf}
%            \fi
%        }
%    }
%}

\usepackage[utf8]{inputenc}
\usepackage{lipsum}

\usepackage{soul,color}

%\usepackage{charter}
\usepackage{xlop}
\usepackage{booktabs}

\def\code#1{\texttt{#1}}
%\usepackage[notref,notcite]{showkeys}
\usepackage{todonotes}
\presetkeys{todonotes}{backgroundcolor=blue!20!white}{} %,inline,fancyline
\setlength{\marginparwidth}{1.5cm}
\def\xhigh{\presetkeys{todonotes}{backgroundcolor=red!20!white,linecolor=red}{}}
\def\xmid{\presetkeys{todonotes}{backgroundcolor=orange!20!white,linecolor=orange}{}}
\def\xlow{\presetkeys{todonotes}{backgroundcolor=green!20!white,linecolor=green}{}}
%\newcommand{\todohigh}[1]{\todo[color=red]{#1}{}}
%\def\todomid#1{\todo[color=orange]{#1}{}}
%\def\todolow#1{\todo[color=green]{#1}{}}

%\usepackage{glossaries}
%\setacronymstyle{long-short}
\usepackage{enumitem}

\newcommand{\hloutlinecolor}{blue}
\newcommand{\hloutlinecolordone}{green}
\newcommand{\hloutlinecolorcurrent}{red}
\newcommand{\ajs}{\color{red}}
\newcommand{\hloutline}[1]{
\noindent\fcolorbox{\hloutlinecolor}{white!90!\hloutlinecolor}{\parbox{\columnwidth}{
\begin{itemize}[leftmargin=*,label={\checkmark}]
#1
\end{itemize}}}
}
\newcommand{\hloutlinedone}[1]{
\noindent\fcolorbox{\hloutlinecolordone}{white!90!\hloutlinecolordone}{\parbox{\columnwidth}{
\begin{itemize}[leftmargin=*,label={\checkmark}]
#1
\end{itemize}}}
}
\newcommand{\hloutlinecurrent}[1]{
\noindent\fcolorbox{\hloutlinecolorcurrent}{white!90!\hloutlinecolorcurrent}{\parbox{\columnwidth}{
\begin{itemize}[leftmargin=*,label={\checkmark}]
#1
\end{itemize}}}
}
\usepackage{flushend}


==> sec/dontForget.tex <==
Writing:
- related work horovod
- avg numbers
*** fix the writing- choose only decentralized

Figures:
- add pics of aggregation patterns

Done
- compare with arxiv msr paper



==> sec/outline.tex <==
- PS has been the historical choice for ML algorithms

- Why PS fits well?
- Using PS was a natural evolution from HDFS in a map reduce
- PS fits well with async training (async SGD) 
- Scale of the jobs were small (input data and parameter size)

Why PS is not sufficient now?
- Incast/outcast
- push for using faster high-performance networks led to the adoption of MPI style communication APIs, which were not a natural fit for PS
- natural solution, AR, not tested or implemented in commodity networks where it can provide significant performance improvement

- Challenges in implementing AR in commodity networks
- Lack of AR support in commodity hardware/spftware stack
- MPI codesigned with topology

- MPI/AR are not fault-tolerant. However, our application as we show can be
- extra load can be 1/(n-1) instead of 1 iteration in PS
- AR only supports synchronous training, async training was the norm before, not anymore

What we do?
- improve network efficiency in graph-based distributed ML models
- show the range of system configs where PS is better, and AR is better. Show AR better in most cases. So we improve AR
- Add AR to the graph model (option for user to switch of AR)
- Improve fault tolerance
- Optimizing AR with knowledge of the underlying model (critical for commodity architecture, not so much for HPC, but wont make HPC performance worse)
- We reduce straggling workers using an online adaptive strategy
- enforce a fixed execution order for consistent iteration time


Sections
Background
Proposed Improvements
System design
Experiments
Discussion
Related Work
Conclusion

Random points:
- large amount of data, ring is way better than anything else including shuffling, halving-doubling


Background
- distributed training , barriers, networking, model-replica

Motivation
- problem metric - network cost, overlap
- transfers in distributed DNN: multiple versions, aggregation
- two ways - centralized --- good overlap, may have bad transfer cost due to unequal load distr, incast/outcast
- decentralized --- better network cost, worse overlap, constraints (ready before start)
look at model
choose the best pattern
optimize overlap



==> sec/title.tex <==
% cAR-ML: Improving Network Efficiency of Distributed Machine Learning in the Cloud
\sysname: Accelerating Distributed Deep Learning with Computation Scheduling
